PROV-IO+: A Cross-Platform Provenance Framework for Scientific Data on HPC Systems

Data provenance, or data lineage, describes the life cycle of data. In scientific workflows on HPC systems, scientists often seek diverse provenance (e.g., origins of data products, usage patterns of datasets). Unfortunately, existing provenance solutions cannot address the challenges due to their incompatible provenance models and/or system implementations. In this paper, we analyze four representative scientific workflows in collaboration with the domain scientists to identify concrete provenance needs. Based on the first-hand analysis, we propose a provenance framework called PROV-IO+, which includes an I/O-centric provenance model for describing scientific data and the associated I/O operations and environments precisely. Moreover, we build a prototype of PROV-IO+ to enable end-to-end provenance support on real HPC systems with little manual effort. The PROV-IO+ framework can support both containerized and non-containerized workflows on different HPC platforms with flexibility in selecting various classes of provenance. Our experiments with realistic workflows show that PROV-IO+ can address the provenance needs of the domain scientists effectively with reasonable performance (e.g., less than 3.5% tracking overhead for most experiments). Moreover, PROV-IO+ outperforms a state-of-the-art system (i.e., ProvLake) in our experiments.

==> 11_biography.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:
%\vspace{-48pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author_photo/runzhou.jpeg}}]{Runzhou Han}
 is a Ph.D. student in the Department of Electrical and Computer Engineering at Iowa State University. He received a MS degree from Boston University and a BS degree from Wuhan Univeristy.
Runzhou Han's research intersts include  large scale storage systems, data provenance and metadata management, and serverless computing. 
\end{IEEEbiography}

% if you will not have a photo at all:
%\vspace{-38pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author_photo/MZ.jpg}}]{Mai Zheng}
 is an Associate Professor in the Dept. of Electrical and Computer Engineering at Iowa State University. He leads the Data Storage Lab to investigate problems of real-world systems that affect data integrity, reproducibility, etc. 
 %His work appeared at storage systems venues (e.g., FAST, SYSTOR, HotStorage, TOS), high-performance computing venues (e.g., HPDC, ICS, TPDS), and other systems venues (e.g., OSDI, ASPLOS, ATC, TOCS). 
 He received the NSF CAREER award in 2020 and Best Paper Honorable Mentions at FAST and HotStorage. Mai received his Ph.D. in Computer Science from The Ohio State University. 
 %For more information, please visit https://www.ece.iastate.edu/~mai/.
\end{IEEEbiography}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage
%\vspace{-40pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author_photo/Suren-Byna.jpg}}]{Suren Byna} 
  is a Professor at  The Ohio State University. He was a Senior Scientist in the Scientific Data Division at Lawrence Berkeley National Lab (LBNL) before joining OSU. His research interests are in scientific data management. More specifically, he's interested in parallel I/O, data management systems for managing scientific data, and heterogeneous computing. 
\end{IEEEbiography}

%\vspace{-38pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author_photo/Houjun-Tang.jpeg}}]{Houjun Tang}
 is currently a Computer Research Scientist in the Scientific Data Management Group at Berkeley Lab. His research interests include data management, storage systems, parallel I/O, and high performance computing. 
\end{IEEEbiography}

%\vspace{-38pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author_photo/Bin-Dong.jpeg}}]{Bin Dong}
  is a Research Scientist in the Scientific Data Division at Lawrence Berkeley National Lab (LBNL). Bin's research interests are in Big scientific data management and analysis, parallel computing, machine learning,  etc.  
Currently, Bin is exploring new and scalable algorithms and data structures for sorting, organizing, indexing, searching, analyzing Big scientific data (mostly as array) with supercomputers. 
\end{IEEEbiography}

%\vspace{-38pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author_photo/Dai-Dong.jpg}}]{Dong Dai}
 is an Assistant Professor in the Computer Science Department at University of North Carolina at Charlotte.  He received his Doctor degree in Computer Science from University of Science and Technology of China (USTC).
His research interests are related to building intelligent infrastructure for high-performance data-intensive systems, including parallel file systems, metadata management, graph storage, scheduling, and ML frameworks.
\end{IEEEbiography}

%\vspace{-38pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author_photo/Chen-Yong.jpg}}]{Yong Chen}
 is a Principal Software Engineer Lead and Architect at Samsung Electronics. 
 %He has worked on storage and distributed systems for more than twenty years. 
 His expertise includes distributed file systems, NVMe/SPDK, RDMA/high-speed transport, high available systems, security, as well as scale-out and high performance computing (HPC) clusters. He has contributed to releasing major software/hardware/systems in storage at Microsoft, Huawei, CNEX Labs and Stellus/Samsung. He earned Ph.D. in Computer Science from Michigan State University.
\end{IEEEbiography}

%\vspace{-38pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author_photo/Dongkyun-Kim.jpeg}}]{Dongkyun Kim}
 is a Senior Staff Engineer within Samsung Neural Processing Lab (NPL), overseeing HW \& SW co-design of HPC computing. He lead technology intelligence group in Samsung Advanced Institute of Technology (SAIT)   to find new technology themes and projects. One of which was the proposal of Neural Processing Unit in 2015, which later became Samsung NPL. He has a Ph.D. in physics from Univ. California, San Diego, and BS/MS in physics from Seoul National University. 
\end{IEEEbiography}

%\vspace{-38pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author_photo/Joseph-Hassoun.jpg}}]{Joseph Hassoun}
 is the Director of the Neural Processing Lab (NPL),
 %at Samsung Advanced Institute of Technology (SAIT), 
 Samsung Electronics. He leads the architecture design of Neural Processing Units (NPUs) which were implemented into the Exynos SOCs and used to produce Galaxy family of products. 
% His career spans Xilinx’s Virtex FPGA architecture, Hewlett-Packard Enterprise’s server architecture, and several start-ups.
Joseph received MS EE degree from Stanford Univ. and BS EE from  Univ. of Michigan. He was awarded 29 patents in the fields of Computer Architecture, Deep Learning, and Circuit Design.
\end{IEEEbiography}

%\vspace{-38pt}
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author_photo/David.jpeg}}]{David Thorsley}
  is a technical lead on the algorithms \& machine learning group within the Samsung SAIT’s Neural Processing Lab, where the team is currently doing research in efficient deep learning and hardware/software co-design. He has a Ph.D. in Electrical Engineering from the University of Michigan and has also published research in fields such as control theory, synthetic biology, and physiology.
%David Thorsley is a technical lead on the algorithms and machine learning group within the Samsung Neural Processing Lab, where the team is currently doing research in efficient deep learning and hardware/software co-design. He has a Ph.D. in Electrical Engineering: Systems from the University of Michigan and has also published research in fields such as control theory, synthetic biology, and physiology.
\end{IEEEbiography}

% if you will not have a photo at all:
%\vspace{-38pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author_photo/matthew.jpeg}}]{Matthew Wolf} is a Senior Principal Engineer at Samsung SAIT's Systems Architecture Lab. He leads the technical space for data management, storage, and middleware for Samsung's next generation HPC systems. Before joining Samsung, he was a Senior Scientist at Oak Ridge National Laboratory (ORNL) and served a variety of leadership roles. Matthew received his Ph.D. from Georgia Institute of Technology.

 %For more information, please visit https://www.ece.iastate.edu/~mai/.
\end{IEEEbiography}



%\begin{IEEEbiography}{James Loo}
%James Loo is a Senior Staff Platform Software Architect at Samsung Research.
%\end{IEEEbiography}



%\begin{IEEEbiography}{Jim Wayda}
%Jim Wayda is a researcher at  the Neural Processing Lab (NPL) at Samsung Advanced Institute of Technology (SAIT), Samsung Electronics.
%\end{IEEEbiography}




% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}

